Competition Report: CHC-COMP-20

CHC-COMP-20 is the third competition of solvers for Constrained Horn Clauses. In this year, 9 solvers participated at the competition, and were evaluated in four separate tracks on problems in linear integer arithmetic, linear real arithmetic, and arrays. The competition was run in the first week of May 2020 using the StarExec computing cluster. This report gives an overview of the competition design, explains the organisation of the competition, and presents the competition results.

==> eptcsdata.tex <==
\providecommand{\firstpage}{197}
\providecommand{\publicationstatus}{L. Fribourg and M. Heizmann (Eds.): VPT/HCVS 2020\\
EPTCS 320, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.320.15}{10.4204/EPTCS.320.15}}
\pdfoutput=1

